Symbol Level Precoding for Systems with Improper Gaussian Interference

This paper focuses on precoding design in multi-antenna systems with improper Gaussian interference (IGI), characterized by correlated real and imaginary parts. We first study block level precoding (BLP) and symbol level precoding (SLP) assuming the receivers apply a pre-whitening filter to decorrelate and normalize the IGI. We then shift to the scenario where the base station (BS) incorporates the IGI statistics in the SLP design, which allows the receivers to employ a standard detection algorithm without pre-whitenting. Finally we address the case where the channel and statistics of the IGI are unknown, and we formulate robust BLP and SLP designs that minimize the worst case performance in such settings. Interestingly, we show that for BLP, the worst-case IGI is in fact proper, while for SLP the worst case occurs when the interference signal is maximally improper, with fully correlated real and imaginary parts. Numerical results reveal the superior performance of SLP in terms of symbol error rate (SER) and energy efficiency (EE), especially for the case where there is uncertainty in the non-circularity of the jammer.

==> arraymac.tex <==
% general purpose macros fo use with LaTeX (or TeX)
\makeatletter
\newfont{\sqi}{cmssqi8}
\newcommand{\IR}{\mbox{$I\!\!R$}}
\newcommand{\IC}{\mbox{$C\!\!\!\!\raisebox{.75pt}{\mbox{\sqi I}}\;\,$}}
\def\defnas{\stackrel{\rm def}{=}}
\newcommand\vdashl{\vdshl{1}{1}}
\newcommand\bvdashl{\vdshl{1.6}{2}}
\newlength{\tmpln}
\newlength{\dshln}
\newcommand{\vdshl}[2]{{\setbox1=\hbox{$[$}\setlength{\tmpln}{#1\ht1}
\advance\tmpln by #1\dp1
\setlength{\dshln}{.111\tmpln}
\newcommand\vs{\vskip .111\tmpln plus 1pt minus 1pt}
\newcommand\vd{\hrule width .4pt height \dshln depth 0pt}
\setbox2=\hbox{
 \vbox to\tmpln{\lineskip 0pt \lineskiplimit-1000pt \baselineskip 0pt
 \vd\vs\vd\vs\vd\vs\vd\vs\vd\vfil}$\;$}
 \lower#2\dp1\copy2
}}
\newcommand\adots{\mathinner{\mskip0mu\raise0pt\vbox{\kern7pt\hbox{.}}\mskip3mu
    \raise4pt\hbox{.}\mskip3mu\raise8pt\hbox{.}\mskip0mu}}
\def\nonumfootnotetext{\xdef \@thefnmark{}\@footnotetext}
\def\ie{{\it i.e.,\ }}
\def\cf{{\it cf.\ }}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\eg{{\it e.g.,\ }}
\def\apriori{{\it a~priori}}
\def\qed{%
   {%
      \unskip
      \nobreak \hfil
      \penalty 50               % TeX should break here if necessary
      \hskip 3em                % mimium amount of distance
      \null \nobreak \hfil
      \qedbox
      \parfillskip=\z@skip
      \finalhyphendemerits=\z@  % no line break at last line of paragraph
      \endgraf                  % don't know what \par is in this moment...
   }}
\def\qedbox{\rule[-1pt]{8pt}{8pt}}\def\QED{\qed}
%\def\beq{\@ifnextchar [{\@tempswatrue\@beq}{\@tempswafalse\@beq[]}}
%\def\@beq[#1]{\begin{equation}\edef\@tmparg{#1}\ifx\@tmparg\@empty \else
%        \label{#1}\fi}
\def\beq[#1]{\begin{equation} \label{#1}}
\newcommand{\eeq}{\end{equation}}
%\def\eeq{\end{equation}}
% \jot 2ex
\newcount\@eqcnt
\newcount\@eqpen
\newif\if@eqnsw\@eqnswtrue
\def\eqnarray{\stepcounter{equation}\let\@currentlabel=\theequation
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@eqncr
$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
  \hskip .6\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip .6\arraycolsep $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\str{\rule[-.6em]{0pt}{2.4em}}
\def\proof{\noindent {\bf Proof:\ }}
\let\pbox=\qed
\def\dag{{\cal y}}
\def\phstar{{\phantom{*}}}
\def\dmax{d_{\rm max}}
\def\vcv{\vdashl\cdots\vdashl}
\def\alphabf{{\boldsymbol \alpha}}
\def\betabf{{\boldsymbol \beta}}
\def\gammabf{{\boldsymbol \gamma}}
\def\deltabf{{\boldsymbol \delta}}
\def\epsilonbf{{\boldsymbol \epsilon}}
\def\epsbf{{\boldsymbol \epsilon}}
\def\zetabf{{\boldsymbol \zeta}}
\def\etabf{{\boldsymbol \eta}}
\def\thetabf{{\boldsymbol \theta}}
\def\iotabf{{\boldsymbol \iota}}
\def\kappabf{{\boldsymbol \kappa}}
\def\lambdabf{{\boldsymbol \lambda}}
\def\mubf{{\boldsymbol \mu}}
\def\nubf{{\boldsymbol \nu}}
\def\xibf{{\boldsymbol \xi}}
\def\pibf{{\boldsymbol \pi}}
\def\varphibf{{\boldsymbol \varphi}}
\def\rhobf{{\boldsymbol \rho}}
\def\sigmabf{{\boldsymbol \sigma}}
\def\taubf{{\boldsymbol \tau}}
\def\taubfh{\hat{\taubf}}
\def\upsilonbf{{\boldsymbol \upsilon}}
\def\phibf{{\boldsymbol \phi}}
\def\chibf{{\boldsymbol \chi}}
\def\psibf{{\boldsymbol \psi}}
\def\omegabf{{\boldsymbol \omega}}
\def\Gammabf{{\boldsymbol \Gamma}}
\def\Thetabf{{\boldsymbol \Theta}}
\def\Lambdabf{{\boldsymbol \Lambda}}
\def\Xibf{{\boldsymbol \Xi}}
\def\Pibf{{\boldsymbol \Pi}}
\def\Sigmabf{{\boldsymbol \Sigma}}
\def\Upsilonbf{{\boldsymbol \Upsilon}}
\def\Phibf{{\boldsymbol \Phi}}
\def\Psibf{{\boldsymbol \Psi}}
\def\Psibar{{\bar{\Psibf}}}
\def\Ebar{{\bar{\Ebf}}}
\def\Omegabf{{\boldsymbol \Omega}}
\def\Deltabf{{\boldsymbol \Delta}}
\def\abf{{\bf a}}
\def\bbf{{\bf b}}
\def\cbf{{\bf c}}
\def\dbf{{\bf d}}
\def\ebf{{\bf e}}
\def\fbf{{\bf f}}
\def\gbf{{\bf g}}
\def\hbf{{\bf h}}
\def\ibf{{\bf i}}
\def\iibf{{\bf ii}}
\def\iiibf{{\bf iii}}
\def\jbf{{\bf j}}
\def\kbf{{\bf k}}
\def\lbf{{\bf l}}
\def\ellbf{{\bf \ell}}
\def\mbf{{\bf m}}
\def\nbf{{\bf n}}
\def\obf{{\bf o}}
\def\peebf{{\bf p}}
\def\qbf{{\bf q}}
\def\rbf{{\bf r}}
\def\sbf{{\bf s}}
\def\tbf{{\bf t}}
\def\ubf{{\bf u}}
\def\vbf{{\bf v}}
\def\wbf{{\bf w}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\zbf{{\bf z}}
\def\rbf{{\bf r}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\Abf{{\bf A}}
\def\Bbf{{\bf B}}
\def\Cbf{{\bf C}}
\def\Dbf{{\bf D}}
\def\Ebf{{\bf E}}
\def\Fbf{{\bf F}}
\def\Gbf{{\bf G}}
\def\Hbf{{\bf H}}
\def\Ibf{{\bf I}}
\def\Jbf{{\bf J}}
\def\Kbf{{\bf K}}
\def\Lbf{{\bf L}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Obf{{\bf O}}
\def\Pbf{{\bf P}}
\def\Qbf{{\bf Q}}
\def\Rbf{{\bf R}}
\def\Sbf{{\bf S}}
\def\Tbf{{\bf T}}
\def\Ubf{{\bf U}}
\def\Vbf{{\bf V}}
\def\Wbf{{\bf W}}
\def\Xbf{{\bf X}}
\def\Ybf{{\bf Y}}
\def\Zbf{{\bf Z}}
\def\sf{\mathsf}
\def\asf{{\sf a}}
\def\bsf{{\sf b}}
\def\csf{{\sf c}}
\def\dsf{{\sf d}}
\def\esf{{\sf e}}
\def\fsf{{\sf f}}
\def\gsf{{\sf g}}
\def\hsf{{\sf h}}
\def\isf{{\sf i}}
\def\iisf{{\sf ii}}
\def\iiisf{{\sf iii}}
\def\jsf{{\sf j}}
\def\ksf{{\sf k}}
\def\lsf{{\sf l}}
\def\ellsf{{\sf \ell}}
\def\msf{{\sf m}}
\def\nsf{{\sf n}}
\def\osf{{\sf o}}
\def\psf{{\sf p}}
\def\qsf{{\sf q}}
\def\rsf{{\sf r}}
\def\ssf{{\sf s}}
\def\tsf{{\sf t}}
\def\usf{{\sf u}}
\def\vsf{{\sf v}}
\def\wsf{{\sf w}}
\def\xsf{{\sf x}}
\def\ysf{{\sf y}}
\def\zsf{{\sf z}}
\def\rsf{{\sf r}}
\def\xsf{{\sf x}}
\def\ysf{{\sf y}}
\def\Asf{{\sf A}}
\def\Bsf{{\sf B}}
\def\Csf{{\sf C}}
\def\Dsf{{\sf D}}
\def\Esf{{\sf E}}
\def\Fsf{{\sf F}}
\def\Gsf{{\sf G}}
\def\Hsf{{\sf H}}
\def\Isf{{\sf I}}
\def\Jsf{{\sf J}}
\def\Ksf{{\sf K}}
\def\Lsf{{\sf L}}
\def\Msf{{\sf M}}
\def\Nsf{{\sf N}}
\def\Osf{{\sf O}}
\def\Psf{{\sf P}}
\def\Qsf{{\sf Q}}
\def\Rsf{{\sf R}}
\def\Ssf{{\sf S}}
\def\Tsf{{\sf T}}
\def\Usf{{\sf U}}
\def\Vsf{{\sf V}}
\def\Wsf{{\sf W}}
\def\Xsf{{\sf X}}
\def\Ysf{{\sf Y}}
\def\Zsf{{\sf Z}}
\def\CRB{{\bf CRB}}
\def\FIM{{\bf FIM}}
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}
\def\xbfhat{\hat{\xbf}}
\def\lambdahat{\hat{\lambda}}
\def\lh{\hat{\lambda}}
\def\dh{\hat{d}}
\def\sh{\hat{s}}
\def\sdhh{\hat{\hat{s}}_d}
\def\wh{\hat{\wbf}}
\def\Phibar{\bar{\Phibf}}
\def\lambdatilde{\tilde{\lambda}}
\def\lambdabfhat{\hat{\lambdabf}}
\def\lambdatbf{{\tilde {\lambdabf}}}
\def\At{{\tilde{\Abf}}}
\def\Bt{{\tilde{\Bbf}}}
\def\Ath{{\hat{\tilde{\Abf}}}}
\def\Gt{{\tilde{\Gbf}}}
\def\Tt{{\tilde{\T}}}
\def\Ah{{\hat{\Abf}}}
\def\Gh{{\hat{\Gbf}}}
\def\Qh{{\hat{\Qbf}}}
\def\Th{{\hat{\T}}}
\def\Uh{{\hat{\U}}}
\def\a{{\abf}}
\def\d{{\dbf}}
\def\s{{\sbf}}
\def\x{{\xbf}}
\def\y{{\ybf}}
\def\at{{\tilde{\abf}}}
\def\bt{{\tilde{\bbf}}}
\def\ah{{\hat{\abf}}}
\def\th{{\theta}}
\def\thh{{\hat{\theta}}}
\def\thi{{\theta_i}}
\def\thih{{\hat{\theta}_i}}
\def\thk{{\theta_k}}
\def\thik{{\hat{\theta}_k}}
\def\ai{{\a(\theta_i)}}
\def\ath{{\a(\theta)}}
\def\aths{{\a^*(\theta)}}
\def\athT{{\a^T(\theta)}}
\def\ais{{\a^*(\theta_i)}}
\def\ait{{\a^T(\theta_i)}}
\def\ak{{\a(\theta_k)}}
\def\aks{{\a^*(\theta_k)}}
\def\akt{{\a^T(\theta_k)}}
\def\thbf{{\thetabf}}
\def\sbft{{\tilde{\sbf}}}
\def\thbft{{\tilde{\thbf}}}
\def\thbfh{{\hat{\thbf}}}
\def\rhobfh{{\hat{\rhobf}}}
\def\thbfhh{{\hat{\hat{\thbf}}}}
\def\etat{{\tilde{\eta}}}
\def\etabft{{\tilde{\etabf}}}
\def\etabfth{{\hat{\tilde{\etabf}}}}
\def\etabfhh{{\hat{\hat{\etabf}}}}
\def\etabfh{{\hat{\etabf}}}
\def\alphabfh{{\hat{\alphabf}}}
\def\Vh{{\hat{V}}}
\def\Vt{{\tilde{V}}}
\def\therr{{\hat{\theta}-\theta}}
\def\therrbf{{\hat{\thetabf}-\thetabf_0}}
\def\therrbfwsf{{\hat{\thetabf}_\WSF-\thetabf_0}}
\def\etaerr{{\hat{\eta}-\eta}}
\def\etaerrbf{{\hat{\etabf}-\etabf_0}}
\def\etabfhat{{\hat{\etabf}}}
\def\ebh{{\etabfhat}}
\def\ebz{{\etabf_0}}
\def\Capo{{\C^{pq}_{a,1}}}
\def\Capt{{\C^{pq}_{a,2}}}
\def\Cesp{{\C_\ES}}
\def\therri{{\thih-\thi}}
\def\therrk{{\thik-\thk}}
\def\Cxik{{\Cbf_{\xi,1}^{ik}}}
\def\CxikT{{\Cbf_{\xi,2}^{ik}}}
\def\Cxpq{{\Cbf_{\xi,1}^{pq}}}
\def\CxpqT{{\Cbf_{\xi,2}^{pq}}}
\def\Cxii{{\Cbf_{\xi,1}^{ii}}}
\def\CxiiT{{\Cbf_{\xi,2}^{ii}}}
\def\Cxi{{\Cbf_{\xi,1}^{i}}}
\def\CxiT{{\Cbf_{\xi,2}^{i}}}
\def\Cx{{\Cbf_{\xi,1}}}
\def\CxT{{\Cbf_{\xi,2}}}
\def\Cmu{{\Cbf_{\MU}}}
\def\Cmuf{{\Cbf_{\MUF}}}
\def\Cmuik{{\Cbf_{\MU,ik}}}
\def\Cwmu{{\Cbf_{\WMU}}}
\def\Cwmuik{{\Cbf_{\WMU,ik}}}
\def\Lsl{{\Lambdabf_s}}
\def\Ls{{\Lambdabf_s}}
\def\Lh{{\hat{\Lambdabf}}}
%\def\Lsh{{\hat{\Lambdabf}_s}}
\def\Lshat{{\Lsh}}
\def\Lnh{{\hat{\Lambdabf}_n}}
\def\Lnhi{{\hat{\Lambdabf}_n^{-1}}}
\def\Lst{{\tilde{\Lambdabf}_s}}
\def\Lnt{{\tilde{\Lambdabf}_n}}
\def\Lt{{\tilde{\Lambdabf}}}
\def\Ltilde{{\Lt}}
\def\Lo{{\overline{\Lambdabf}}}
\def\Cx{{\Cbf_{\xi,1}}}
\def\CxT{{\Cbf_{\xi,2}}}
\def\pht{{\tilde{\phi}}}
\def\gt{{\tilde{g}}}
\def\xt{{\tilde{x}}}
\def\yt{{\tilde{y}}}
\def\xbft{{\tilde{\xbf}}}
\def\ybft{{\tilde{\ybf}}}
\def\gtogk{{{\gt_k}\over{g_k}}}
\def\atoak{{{\tilde{a}_k}\over{a_k}}}
\def\w{{\omega}}
\def\EEP{{\Ebar_W^*\Ebar_W \Pbf_{\bar{\Psibf}^*}^\perp}}
\def\EPp{{\Ebar_W \P_{\bar{\Psibf}^*}^\perp}}
\def\EP{{\Ebar_W \P_{\bar{\Psibf}^*}}}
\def\Eyha{{{\hat{\Ebf}}_y^\phstar}}
\def\LPbar{{\Psibar^*(\Psibar\Psibar^*)^{-1}}}
\def\PPbar{{\Psibar^*(\Psibar\Psibar^*)^{-1}\Psibar}}
\def\ppij{{{\partial}\over{\Psibf_{ij}}}}
\def\Pho{{{\hat{\Psibf}}_1}}
\def\Phw{{{\hat{\Psibf}}_2}}
\def\Phh{{{\hat{\Psibf}}_3}}
\def\pho{{{\hat{\psibf}}_1}}
\def\phw{{{\hat{\psibf}}_2}}
\def\phh{{{\hat{\psibf}}_3}}
\def\Pbh{{{\hat{\Psibar}}}}
\def\Pti{{{\tilde{\Psibf}}_i}}
\def\Pbi{{{\hat{\Psibf}}_i}}
\def\pto{{{\tilde{\psibf}}_1}}
\def\ptw{{{\tilde{\psibf}}_2}}
\def\pth{{{\tilde{\psibf}}_3}}
\def\Pto{{{\tilde{\Psibf}}_1}}
\def\Ptw{{{\tilde{\Psibf}}_2}}
\def\Pth{{{\tilde{\Psibf}}_3}}
\def\Pbt{{{\tilde{\Psibar}}}}
\def\En{{\Ebf_n}}
\def\Es{{\Ebf_s}}
\def\Ens{{\Ebf_n^*}}
\def\Ess{{\Ebf_s^*}}
\def\Eh{{\hat{\E}}}
\def\Et{{\tilde{\E}}}
\def\Ehh{{\hat{\hat{\E}}}}
\def\Ett{{\tilde{\tilde{\E}}}}
\def\Eshh{{\hat{\hat{\Ebf}}_s}}
\def\Enhh{{\hat{\hat{\Ebf}}_n}}
\def\Eshhs{{\hat{\hat{\Ebf}}_s^*}}
\def\Enhhs{{\hat{\hat{\Ebf}}_n^*}}
\def\Ent{{{\tilde{\Ebf}}_n}}
\def\Est{{{\tilde{\Ebf}}_s}}
\def\Entt{{\tilde{\tilde{\Ebf}}_n}}
\def\Estt{{\tilde{\tilde{\Ebf}}_s}}
\def\Entts{{\tilde{\tilde{\Ebf}}_n^*}}
\def\Estts{{\tilde{\tilde{\Ebf}}_s^*}}
\def\Ents{{{\tilde{\Ebf}}_n^*}}
\def\Ests{{{\tilde{\Ebf}}_s^*}}
\def\Enh{{\hat{\Ebf}_n}}
\def\Esh{{\hat{\Ebf}_s}}
\def\Enhs{{\hat{\Ebf}_n^*}}
\def\Eshs{{\hat{\Ebf}_s^*}}
\def\Eshz{{\hat{\Ebf}_0}}
\def\Esho{{\hat{\Ebf}_1}}
\def\Eshp{{\hat{\Ebf}_{p-1}}}
\def\EEs{{\Ebf_s^{}\Ebf_s^*}}
\def\EEsh{{\hat{\Ebf}_s^{}\hat{\Ebf}_s^*}}
\def\EEn{{\Ebf_n^{}\Ebf_n^*}}
\def\EEnh{{\hat{\Ebf}_n^{}\hat{\Ebf}_n^*}}
\newcommand{\ENEN}{\mbox{$\hat{\Ebf}_n^{}\hat{\Ebf}_n^*$}}
\def\EWE{{\Ebf_s^{}\Wbf\Ebf_s^*}}
\def\EWEh{{\hat{\Ebf}_s^{}\Wbf\hat{\Ebf}_s^*}}
\def\EWsEh{{\hat{\Ebf}_s^{}\Wbf_s^{}\hat{\Ebf}_s^*}}
\def\EWchEh{{\hat{\Ebf}_s^{}\hat{\Wbf}_c^{}\hat{\Ebf}_s^*}}
\def\EWot{{\Ebf_s \Wbf^{\half}}}
\def\EWoth{{\hat{\Ebf}_s^{} \Wbf^{\half}}}
\def\EWchoth{{\hat{\Ebf}_s^{} \hat{\Wbf}_c^{\half}}}
\def\et{{\tilde{\ebf}}}
\def\eh{{\hat{\ebf}}}
\def\ett{{\tilde{\tilde{\ebf}}}}
\def\ehh{{\hat{\hat{\ebf}}}}
\def\Wcot{{\Wbf_c^{\half}}}
\def\Wrot{{\Wbf_r^{\half}}}
\def\Deltaeq{{\stackrel{\Delta}{=}}}
\def\A{{\Abf}}
\def\B{{\Bbf}}
\def\C{{\Cbf}}
\def\D{{\Dbf}}
\def\E{{\Ebf}}
\def\F{{\Fbf}}
\def\G{{\Gbf}}
\def\H{{\Hbf}}
\def\I{{\Ibf}}
\def\It{{\tilde{\Ibf}}}
\def\J{{\Jbf}}
\def\K{{\Kbf}}
\def\L{{\Lbf}}
\def\M{{\Mbf}}
\def\N{{\Nbf}}
\def\P{{\Pbf}}
\def\Q{{\Qbf}}
\def\R{{\Rbf}}
\def\S{{\Sbf}}
\def\T{{\Tbf}}
\def\U{{\Ubf}}
\def\V{{\Vbf}}
\def\W{{\Wbf}}
\def\X{{\Xbf}}
\def\Y{{\Ybf}}
\def\Z{{\Zbf}}
\def\SNR{{\mbox{\rm SNR}}}
\def\ssSigma{{\scriptscriptstyle \Sigma}}
\def\CB{{\scriptscriptstyle CB}}
\def\CML{{\scriptscriptstyle CML}}
\def\UML{{\scriptscriptstyle UML}}
\def\DML{{\scriptscriptstyle DML}}
\def\SML{{\scriptscriptstyle SML}}
\def\ML{{\scriptscriptstyle ML}}
\def\MD{{\scriptscriptstyle MD}}
\def\MU{{\scriptscriptstyle MU}}
\def\MUF{{\scriptscriptstyle MUF}}
\def\MUD{{\scriptscriptstyle MUD}}
\def\MUDc{{\scriptscriptstyle MUDc}}
\def\WMU{{\scriptscriptstyle WMU}}
\def\MO{{\scriptscriptstyle MO}}
\def\ES{{\scriptscriptstyle ES}}
\def\MSE{{\scriptscriptstyle MSE}}
\def\LS{{\scriptscriptstyle LS}}
\def\TLS{{\scriptscriptstyle TLS}}
\def\BF{{\scriptscriptstyle BF}}
\def\FS{{\scriptscriptstyle FS}}
\def\AR{{\scriptscriptstyle AR}}
\def\WSF{{\scriptscriptstyle WSF}}
\def\OSF{{\scriptscriptstyle OSF}}
\def\SSF{{\scriptscriptstyle SSF}}
\def\RSF{{\scriptscriptstyle RSF}}
\def\NSF{{\scriptscriptstyle NSF}}
\def\MAP{{\scriptscriptstyle MAP}}
\def\OPT{{\scriptscriptstyle OPT}}
\def\FA{{\scriptscriptstyle FA}}
\def\SSE{{\scriptscriptstyle SSE}}
\def\LCMV{{\scriptscriptstyle LCMV}}
\def\SC{{\scriptscriptstyle SC}}
\def\WLS{{\scriptscriptstyle WLS}}
\def\aQa{{\abf^*\Qbf^{-1}\abf}}
\def\dQa{{\dbf^*\Qbf^{-1}\abf}}
\def\aQd{{\abf^*\Qbf^{-1}\dbf}}
\def\dQd{{\dbf^*\Qbf^{-1}\dbf}}
\def\zerobf{{\bf 0}}
\def\onebf{{\bf 1}}
\def\half{{{1}\over{2}}}
\def\halfT{{{*}\over{2}}}
\def\jhalf{{{j}\over{2}}}
\def\mjhalf{{{-j}\over{2}}}
\def\mhalf{{-\half}}
\def\Rss{{\Rbf_{ss}}}
\def\Rssi{{\Rbf_{ss}^{-1}}}
\def\Rsst{{\R_{\sbf\tilde{s}}}}
\def\RsstH{{\R_{\sbf\tilde{s}}^*}}
\def\Rssb{{\Rbf_{\sbf\sbf}}}
\def\Rssbi{{\Rbf_{\sbf\sbf}^{-1}}}
\def\Rssd{{\Rbf_{\sbf s_d}}}
\def\RssdH{{\Rbf_{\sbf s_d}^*}}
\def\Rssh{{\hat{\Rbf}_{ss}}}
\def\Rxs{{\Rbf_{xs}}}
\def\Rxsb{{\Rbf_{\xbf\sbf}}}
\def\RxsH{{\Rbf_{x\sh}}}
\def\Rxx{{\Rbf_{xx}}}
\def\Rxxb{{\Rbf_{\xbf\xbf}}}
\def\Rxxbi{{\Rbf_{\xbf\xbf}^{-1}}}
\def\Rxxh{{\hat{\Rbf}_{xx}}}
\def\Ryyh{{\hat{\Rbf}_{yy}}}
\def\Rysh{{\hat{\Rbf}_{ys}}}
\def\Rxxo{{\Rbf_{xx0}}}
\def\Rzz{{\Rbf_{zz}}}
\def\Rzzh{{\hat{\Rbf}_{zz}}}
\def\Rh{{\hat{\R}}}
\def\Rhi{{\hat{\R}^{-1}}}
\def\Rhat{{\Rh}}
\def\Sh{{\hat{\S}}}
\def\St{{\tilde{\S}}}
\def\Xh{{\hat{\X}}}
\def\Xt{{\tilde{\X}}}
\def\Ad{{\A^\dag}}
\def\Adt{{\A^{\dag *}}}
\def\Sd{{\S^\dag}}
\def\Sdt{{\S^{\dag *}}}
\def\Th{{\hat{\T}}}
\def\Wh{{\hat{\W}}}
\def\Wt{{\tilde{\W}}}
\def\Rt{{\tilde{\R}}}
\def\Rhs{{\Rh^{}_\Sigma}}
%%\def\Rs{{\R^{}_\Sigma}}
\def\PAp{{\P_A^\perp}}
\def\PA0p{{\P_{A_0}^\perp}}
\def\PAs{{\P^{}_{{\Sigma^\mhalf A}}}}
\def\PAps{{\P^\perp_{{\Sigma^\mhalf A}}}}
\def\Pas{{\P^{}_{{\Sigma^\mhalf a(\theta)}}}}
\def\Paps{{\P^\perp_{{\Sigma^\mhalf a(\theta)}}}}
\def\DA{{\Delta\A}}
\def\Dt{{\Deltabf}}
\def\Sgbf{{\Sigmabf}}
\def\Sgbfh{{\hat{\Sigmabf}}}
\def\Sgbft{{\tilde{\Sgbf}}}
\def\Sgot{{\Sgbf^\mhalf}}
\def\Sgotm{{\Sgbf^\half}}
\def\Sgi{{\Sgbf^{-1}}}
\def\sg{{\sigma}}
\def\snt{{\sigma_n^2}}
\def\sdt{{\sigma_d^2}}
\def\snth{{\hat{\sigma}_n^2}}
\def\sat{{\sigma_a^2}}
\def\stwo{{\sigma^2}}
\def\s2h{{\hat{\sigma}^2}}
\def\Trss{{\Tr(\Rss)}}
\def\real{{\mbox{\rm real}}}
\def\imag{{\mbox{\rm imag}}}
\def\diag{{\mbox{\rm diag}}}
\def\spann{{\mbox{\rm span}}}
\def\Re{{\mbox{\rm Re}}}
\def\Im{{\mbox{\rm Im}}}
\def\Tr{{\mbox{\rm Tr}}}
\def\vecc{{\mbox{\rm vec}}}
\def\det{{\mbox{\rm det}}}
\def\rank{{\mbox{\rm rank}}}
\def\ba{\begin{array}}
\def\ea{\end{array}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\beas{\begin{eqnarray*}}
\def\eeas{\end{eqnarray*}}
\newcommand{\onempphp}[1]{
  \iftwocol  \unitlength .45pt
    \[\begin{picture}(440,320)(0,0)
     \special{psfile=#1 hscale=45 vscale=45 voffset=-10}%
    \end{picture}\]
  \else  \unitlength .8pt
    \begin{center} \begin{picture}(440,290)(0,0)
     \special{psfile=#1 hscale=.90 vscale=.80 hoffset=-20 voffset=-25}%
    \end{picture} \end{center}
  \fi
}

% Local Variables:
% mode: plain-tex
% TeX-master: t
% End:

